I Can't Believe There's No Images! Learning Visual Tasks Using only Language Supervision

Many high-level skills that are required for computer vision tasks, such as parsing questions, comparing and contrasting semantics, and writing descriptions, are also required in other domains such as natural language processing. In this paper, we ask whether it is possible to learn those skills from text data and then transfer them to vision tasks without ever training on visual training data. Key to our approach is exploiting the joint embedding space of contrastively trained vision and language encoders. In practice, there can be systematic differences between embedding spaces for different modalities in contrastive models, and we analyze how these differences affect our approach and study strategies to mitigate this concern. We produce models using only text training data on four representative tasks: image captioning, visual entailment, visual question answering and visual news captioning, and evaluate them on standard benchmarks using images. We find these models perform close to models trained on images, while surpassing prior work for captioning and visual entailment in this text-only setting by over 9 points, and outperforming all prior work on visual news by over 30 points. We also showcase a variety of stylistic image captioning models that are trained using no image data and no human-curated language data, but instead using readily-available text data from books, the web, or language models.

==> bk/introduction_v0.tex <==
\section{Introduction}
% Chris
In this paper we consider a \textit{cross-modal} transfer learning setting where a model is trained to complete a task using natural language training data, and then tested on its ability to complete that same task with visual inputs instead of text.
This is an inherently challenging task due to the extreme train-test distribution shift, however it is made possible by the fact the skills that need to be learned during training, such as parsing and understanding an input question, comparing and contrasting different semantic meanings, or constructing outputs in a particular format, are identical when applied to the semantic content of either text and visual input. Therefore it is possible to learn those skills in a modality-general from the text training data and apply them directly to images.


Accomplishing this goal raises the possibility of training certain kinds of computer vision models using pure text data, which has many potential applications. Text data is often easier to obtain then visual data because it can be directly authored by annotators, or even by large language model such a GPT-3~\cite{}. As a result gathering text training to teach a model a particular skill can be far less expensive then gathering and annotating images for the same purpose. 
It also creates the possibility of directly use existing natural language datasets to help train computer vision models.
We demonstrate these applications by using our method to train several stylistic captioning models without using any annotated images.
% This setting also mimics the ability of humans to learn practical skill from natural language sources (e.g., ). 

Our key method for completing this goal is to leverage visual and language (V\&L) models trained with contrastive pre-training~\cite{}. Contrastive pre-training trains models to embed text and images into vectors such that the text and image vectors of paired images and text are close together, and vectors for randomly select images and captions are far apart. These method have been used at very large scales~\cite{}, and have been shown to learn visual representations that effectively encode a wide range of visual concepts. Although this loss was originally intended for representation learning and zero-shot evaluation, here we show it can be also used for cross-modal transfer.

An outline of our method is show in Figure~\ref{fig:method}. During training the text input are encoded using the (frozen) text encoder for V\&L model and as feature for the model. During testing, the visual input is embedded with image encoder used in place of the text embedding. Because these encoders were explicitly trained to produce embeddings that encode semantics in similar way, learning to read and process the text embeddings will naturally translate to the ability to read and process the image embeddings.

One difficulty with this approach is that, while vectors produced by contrastive models do share some structure between modalities, there can still be some significant differences between image and text vectors~\cite{}. We propose several solutions including the used of trained adapter to better align the vectors, and adding Gaussian noise to the text vector during training.


\begin{figure}[]
    \centering
    \textit{Teaser diagram showing how the method works, or do we want a two-column figure above the abstract showing the cations?}
    \caption{Cross-modal transfer}
    \label{fig:method}
\end{figure}

We evaluate how effective this approach is on captioning, visual question answers (VQA), and visual entailment. In each case we train model for the task using only text data -- typically using a caption describing a scene as a stand in for an image, and then test the model when using real images. We find training on pure text data results in model\textit{result sentence}. We also show that the use of adapters \textit{mention some ablation results}.

We demonstrate an application of this method by applying our model to learn stylistic captions. We gather text-only captions from several source (....) as examples of what style captions should have, but without gathering any corresponding images. We then train models on these text-only sources, and demonstrate they can produce accurate and stylistic correct captions for images.

\begin{figure*}
    \centering
    \textit{Figure showing stylistic captions}
    \caption{Cross-modal transfer}
    \label{fig:cptions}
\end{figure*}



% In this paper, we study a setting where a model must learn to solve a task in one modality even though the training data for that task is in a different modality.
% This can be viewed as an extreme case of transfer learning -- models must understand how skills learned from the training data apply to very different kinds of inputs that contain a new modality.
% We focus in particular on training on text training and transferring to visual input, which is important due to the relative ease in which text data can be gathered, and mimics how humans can learn practical skill from natural language (e.g., by reading text books or instruction manuals).

% While humans demonstrate this ability routinely, for example learning real-life skills from text books or instruction manuals, this is challenging for AIs due to the need to understand how the two modalities relate without direction supervision.

